Boosting Visual Recognition in Real-world Degradations via Unsupervised Feature Enhancement Module with Deep Channel Prior

The environmental perception of autonomous vehicles in normal conditions have achieved considerable success in the past decade. However, various unfavourable conditions such as fog, low-light, and motion blur will degrade image quality and pose tremendous threats to the safety of autonomous driving. That is, when applied to degraded images, state-of-the-art visual models often suffer performance decline due to the feature content loss and artifact interference caused by statistical and structural properties disruption of captured images. To address this problem, this work proposes a novel Deep Channel Prior (DCP) for degraded visual recognition. Specifically, we observe that, in the deep representation space of pre-trained models, the channel correlations of degraded features with the same degradation type have uniform distribution even if they have different content and semantics, which can facilitate the mapping relationship learning between degraded and clear representations in high-sparsity feature space. Based on this, a novel plug-and-play Unsupervised Feature Enhancement Module (UFEM) is proposed to achieve unsupervised feature correction, where the multi-adversarial mechanism is introduced in the first stage of UFEM to achieve the latent content restoration and artifact removal in high-sparsity feature space. Then, the generated features are transferred to the second stage for global correlation modulation under the guidance of DCP to obtain high-quality and recognition-friendly features. Evaluations of three tasks and eight benchmark datasets demonstrate that our proposed method can comprehensively improve the performance of pre-trained models in real degradation conditions. The source code is available at https://github.com/liyuhang166/Deep_Channel_Prior

==> Figure/Sup_generator.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.95\linewidth]{Figure/Visio-Fig9-Generator.pdf}
\caption{Different generator structures are used in various tasks.}
\label{fig:sup_generator}
\end{figure}

==> Figure/Sup_gram.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\linewidth]{Figure/Visio-Fig8-Gram.pdf}
\caption{Deep Channel Prior is also verified in ResNet50.}
\label{fig:sup_gram}
\end{figure}

==> Sec/4_exp_1.tex <==

\section{Experiments}
\label{section:exps}
% In this section, we first introduce the employed 8 datasets, as well as the experimental details. Subsequently, we conduct a comprehensive ablation study for our two-stage training strategy. Finally, the quantitative and qualitative results on classification, detection and segmentation are reported to demonstrate the effectiveness of our method.
\subsection{Implementation Details}
\textbf{Datasets.} We conduct extensive experiments for evaluating our proposed DCP on three kinds of high-level vision tasks, including image classification, object detection, and semantic segmentation. Specifically, we perform evaluations on one large synthetic baseline dataset and seven real-world degradation datasets. \textbf{More details about the datasets can be found in supplementary material.}
% Tab. \ref{tab:datasets} provides a summary of crucial statistics for the employed datasets. 

\textbf{Training setting.} We employ pre-trained VGG16 \cite{simonyan2014very}, ResNet50 \cite{he2016deep}, YOLOv5 \cite{redmon2016you}, and DeepLabv3+ \cite{chen2018encoder} as the baseline models. The DCP is trained for 200 epochs using Adam optimizer with a batch size of 5. The initial learning rate of generators and discriminators are set to 2e-4 and 1e-4, respectively. The learning rate is multiplied by 0.1 every 10 epochs. All experiments are run on Nvidia A100 GPU. \textbf{More details about the settings of each UIR method can be found in the supplemental material}.
% In this paper, we mainly compare unsupervised image restoration (UIR) and unsupervised domain adaptation (UDA) methods. For synthetic sets, 1,200 randomly selected unpaired images are used to train UIR methods, while 10 images per class form a 10K-sized unpaired set for UDA methods. In the case of real sets, we respectively select 500 unpaired images from Haze-20 \cite{pei2018does}, ExDARK \cite{loh2019getting}, and their corresponding clear sets for training UIR methods, and the respective weights are used for testing across various tasks. Notably, our DCP is trained using 100 unpaired images in all tasks, showcasing its robustness to data quantity, as detailed in Section \ref{ablation}.

\input{Table/ClassificationReal}
\subsection{Low-Quality Image Classification}
\textbf{Quantitative Results.}
To fully verify the effectiveness and generality of DCP, we compare it with 15 kinds of UIR and UDA methods. We conduct the evaluation on one large-scale synthetic dataset (\emph{i.e.}, ImageNet-C \cite{hendrycks2019benchmarking}) and two real degradation datasets(\emph{i.e.}, Haze-20 \cite{pei2018does} and ExDark \cite{loh2019getting}). For ImageNet-C, we choose fog and motion blur conditions for evaluation. As can be seen from Tab. \ref{tab:cls_syn} and Tab. \ref{tab:cls_real}, our proposed method significantly surpasses the UIR and UDA methods in terms of classification accuracy on synthetic degradation datasets. And the UDA methods as the general generalization means, struggle to discern specific degradation types, leading to universally lower performance compared to UIR methods. In addition, since they rely on unpaired but semantic-aligned images for retraining, which is not suitable for real-world applications, we mainly focus on comparison with the UIR methods on real datasets. Continuing, when it comes to real foggy and dark conditions, the improvement of UIR methods is also limited, while our approach can also improve the accuracy of the pre-trained network significantly. For example, on the Haze-20 dataset, the best-performing D4 \cite{yang2022D4} improves ResNet50 by only 0.3\%, while our method can improve by 9.4\%. Similar conclusions can be found on ExDark dataset. All this demonstrates that DCP effectively boosts the performance of pre-trained models in real degradation conditions. 

\input{Figure/Features}

\textbf{Feature Visualization.} To demonstrate the performance of DCP in feature correction, we visualize the feature maps of different methods of real foggy and dark images as shown in Fig. \ref{fig:features}. It can be seen that degradation cues will lead to varying degrees of degradation in the discriminative structures of features, causing content loss and introducing additional artifacts, \emph{e.g.}, cars vanishing in fog and rooms submerged in dark condition. While UIR methods can restore certain structural information in images, they do not consistently enhance the discriminative feature responses of objects. For instance, RefineDNet 
\cite{zhao2021refinednet} and D4 \cite{yang2022D4} can only partially enhance local areas in features, leaving other areas still in haze. Besides, ZeroDCE \cite{guo2020zero} and NeRCo \cite{yang2023implicit} introduce more noise to the dark-shrouded areas, \emph{i.e.}, artifacts. As a contrast, our method significantly boosts the feature responses in the discriminative regions of objects, not only achieving effective restoration of latent content but also suppressing additional artifacts. It demonstrates that our UFEM is robust and applicable to real-world scenarios.


\subsection{Foggy Object Detection}
\textbf{Quantitative Results.}
Compared to image recognition, object detection require both identification and spatial localization of objects, demanding greater completeness and richness in feature content. To further validate the effectiveness of UFEM in feature content restoration, we conduct experimental verification on two real foggy object detection datasets (\emph{i.e.}, RTTS \cite{li2018benchmarking} and DAWN \cite{kenk2020dawn}) and compare it with five SOTA UIR methods. As reported in Tab. \ref{tab:det}, our DCP method exhibits consistent improvements in performance across two real foggy scenarios, outperforming all five UIR methods. This demonstrates that our DCP can more accurately restore the content and details of degraded image features, which, in turn, facilitates improved object recognition and localization within detection networks.

\input{Table/DetectionResult}
\input{Figure/GradCAM}

\textbf{Grad-CAM Attention Visualization.} We next compare the contribution of our UFEM and the UIR methods in accurately drawing the attention of detector leveraging gradCAMs \cite{selvaraju2017grad}. Here, we only present visualization of the optimal UIR method, and \textbf{more results can be found in supplementary materials.} As shown in Fig. \ref{fig:gradcam}, the SLP \cite{ling2023single} fail to effectively guide the detector to focus more accurately on the discriminative regions of the image. This, in turn, results in missed and false detections by the detector, such as the inability to accurately detect the looming riders in fog and the erroneous focus on background areas like the sky and tree trunks. As a contrast, our UFEM better enhances the discriminative regions surrounding the objects compared to UIR methods, allowing the coupled detector to attentively focus and predict the correct category and spatial location of objects. This demonstrates the recognition-friendly property of our UFEM for deep neural networks.

% \textbf{Grad-CAM Attention Visualization.} We next compare the contribution of our DCP and the UIR methods in accurately drawing the attention of detector leveraging gradCAMs \cite{selvaraju2017grad}. As shown in Fig. \ref{fig:gradcam}, the UIR methods fail to effectively guide the detector to focus more accurately on the discriminative regions of the image. This, in turn, results in missed and false detections by the detector, such as the inability to accurately detect the looming riders in fog and the erroneous focus on background areas like the sky and tree trunks. While certain UIR methods (like SNSPGAN \cite{wang2022cycle} and SLP \cite{ling2023single}) can promote the coupled detector to better focus on objects in the images, they still introduce additional erroneous attention. D4 \cite{yang2022D4} can avoid the above issue but still results in missed attention on objects in the haze, such as the person on the far left in the woods. As a contrast, our DCP better enhances the discriminative regions surrounding the objects compared to UIR methods, allowing the coupled detector to attentively focus and predict the correct category and spatial location of objects. This demonstrates the efficiency and recognition-friendly properties of our DCP for deep neural networks.

\subsection{Nighttime Semantic Segmentation}
\textbf{Quantitative Results.}
Semantic segmentation relies on the local consistency of the image to perform pixel-level classification for each point \cite{chen2018encoder}. However, the introduction of degradation cues will disrupt the image's statistical and structural characteristics, posing challenges to pre-trained networks for achieving high-precision semantic segmentation. To confirm the accuracy of UFEM in local feature content restoration, we conduct experiments on three real low-light segmentation datasets (\emph{i.e.}, ACDC Nighttime \cite{sakaridis2021acdc}, Dark\_Zurich \cite{sakaridis2019guided}, and Nighttime Driving \cite{dai2018dark}), and compare it with five advanced UIR methods. As reported in Tab. \ref{tab:seg}, a remarkable observation is that all UIR-based enhancement suffer a significant degradation in performance rather than improvement. In stark contrast, our method consistently achieves a performance boost across all three real low-light datasets, exceeding UIR methods by \textbf{7.5$\sim$10.1\%}. These results validate the effectiveness of our method in restoring the local consistency of degraded features, affirming its generality in handling complex tasks.

\input{Table/SegmentationResult}
\input{Figure/Segmentation}

\textbf{Semantic Segmentation Visualization.} We finally present a qualitative comparison of our UFEM and other UIR methods. As shown in Fig. \ref{fig:segmentation}, our method obviously generates more accurate segmentation for both distant and dense objects in the dark, such as a row of bicycles parked side by side and a car traveling in the distance. All these results affirm the efficacy of our method across various degradation scenarios and tasks. Nonetheless, there is still room for further advancement, particularly in nighttime semantic segmentation, which will be the focus of our upcoming work.

\input{Table/Ablation}
\input{Figure/Datanum}

\subsection{Ablation Study}
\label{ablation}
% In this section, we perform comprehensive ablation studies in two recognition models on the benchmark of ImageNet-C to demonstrate the effectiveness of each component. 
\textbf{Effectiveness of the Multi-adversarial Mechanism.} Firstly, to verify the benefits of multi-adversarial mechanism in Stage-1, we design several variants in Tab. \ref{tab:multidis}. Among them, “1D”, “2D”, and “3D” refer to different numbers of discriminators in DPL. As we can see, equipping deep networks with more discriminators tends to yield better performance than the baseline. However, the gains diminish with an increasing number of discriminators, approaching saturation. And more discriminators bring heavy parameters and computational complexity. Therefore, in this paper, we adopt the “3D” for multi-scale discrimination, effectively addressing challenges posed by sparsity and preventing error accumulation in feature propagation.
% in terms of Top-1 Accuracy of VGG16 on Fog-3. Similar trends are also observed in Fog-1 and Fog-5. This highlights the effectiveness of incorporating discriminators in the post-feature translation layers, which introduces stability and recognition-friendly characteristics to the translated features during deep-layer propagation, thereby significantly improving accuracy.

\textbf{Effectiveness of the Two-stage Training Strategy.} We next conduct an ablation study to analyze the contribution of the two-stage training 
mechanism. As reported in Tab. \ref{tab:twostage}, employing only Stage-1 or Stage-2 leads to some improvement in most cases, indicating the effectiveness of each stage in our method. \textcolor{red}{In addition, Stage-1 generally outperforms Stage-2, highlighting the necessity of initial content restoration.} However, both above fall significantly short of our two-stage correction, indicating that sequentially performing content restoration and channel correlation modulation under DCP guidance is more beneficial for unsupervised feature correction.
% the UFEM only with Stage-1 outperforms baseline by \textbf{17.0\%/14.7\%}, \textbf{1.36\%/2.72\%}, and \textbf{11.4\%/4.6\%} of VGG16 and ResNet50 on Fog-5, Contrast-5 and Motion blur-5, respectively. Moreover, by integrating the training of Stage-2 into UFEM, significant accuracy improvements of \textbf{26.1\%/18.3\%}, \textbf{12.0\%/2.99\%}, and \textbf{6.99\%/5.3\%} are achieved compared to the baseline, and impressive accuracy improvements of \textbf{9.1\%/3.6\%}, \textbf{10.6\%/0.27\%}, and \textbf{3.9\%/0.7\% } are also achieved compared to only Stage-1. The remarkable results reveal the effectiveness of our two-stage training strategy in addressing the challenge of unpaired feature enhancement.

\textbf{Insensitivity of Training Set Scale.} In the end, considering the challenge of collecting large-scale degraded images in real-world, we conduct the data sensitivity experiments by training the UFEM with different numbers of images as shown in Fig. \ref{}. We can observe that our method exhibits significant improvements across various data sizes, even only a few dozen unpaired images are utilized for training, which  demonstrates the practicality of our approach in real-world environments. In this paper, we use 100 pairs of unpaired images to train our UFEM by default.



% Particularly, employing a smaller dataset size (\emph{e.g.}, 80, 100) for training may result in higher performance compared to utilizing a larger dataset size (\emph{e.g.}, 200, 400). Therefore, in all experiments across various tasks, our DCP is trained with a minimal dataset of 100 unpaired images, showcasing its effectiveness with exceptionally low data requirements in real-world scenarios.
% we explore the effect of the training set scale on the performance of DCP. We train DCP with different numbers of unpaired images from Fog-3 of ImageNet-C, \emph{i.e.}, 20, 40, 60, 80, 100, 200, 400, 600, 800, 1,000. The detailed results of the two stages are shown in Fig. \ref{datanum}. As we can see, the two-stage performance of DCP on degraded images  . Particularly, concerning the performance of Stage-2, employing a smaller dataset size (\emph{e.g.}, 80, 100) for training may result in higher performance compared to utilizing a larger dataset size (\emph{e.g.}, 800, 1,000). Even under the extreme settings that only \textbf{20} unpaired images are available for training, our DCP can still boost the accuracy of VGG16 on Fog-5 from \textbf{17.5\%} to \textbf{32.9\%}.



==> Table/ClassificationSynthetic-Blur-Contrast.tex <==

\begin{table*}[htbp]
    \centering
    \caption{The comparisons of our proposed UFEM with Unsupervised Image Restoration (UIR) and Unsupervised Domain Adaption (UDA) methods under three different degradation types, \emph{i.e.}, Motion Blur and Low Contrast. Each corruption type contains 5 severity levels.}
    \label{tab:blur_contrast}
    \resizebox{\textwidth}{!}{
    \renewcommand\arraystretch{1.2}
    \begin{tabular}{lcccccccccccc}
    \Xhline{1.5pt}
                                  &                                  & \multicolumn{1}{c||}{}                                & \multicolumn{5}{c||}{\textbf{Top-1 Accuracy of VGG16 (\%)}}                                                                                                                                                                                                                                                                                 & \multicolumn{5}{c}{\textbf{Top-1 Accuracy of ResNet50 (\%)}}                                                                                                                                                                                                                                                        \\ \cline{4-13} 
\multirow{-2}{*}{\textbf{Method}} & \multirow{-2}{*}{\textbf{Venue}} & \multicolumn{1}{c||}{\multirow{-2}{*}{\textbf{Type}}} & \multicolumn{1}{c|}{\textbf{Level-1}}                           & \multicolumn{1}{c|}{\textbf{Level-2}}                           & \multicolumn{1}{c|}{\textbf{Level-3}}                            & \multicolumn{1}{c|}{\textbf{Level-4}}                            & \multicolumn{1}{c||}{\textbf{Level-5}}                           & \multicolumn{1}{c|}{\textbf{Level-1}}                           & \multicolumn{1}{c|}{\textbf{Level-2}}                           & \multicolumn{1}{c|}{\textbf{Level-3}}                           & \multicolumn{1}{c|}{\textbf{Level-4}}                           & \textbf{Level-5}                           \\ \hline

\multicolumn{13}{c}{\cellcolor[HTML]{EAEAEA}\textbf{Degradation Type: Motion Blur} (\textbf{100} unpaired images for UFEM, \textbf{1200} unpaired images for UIR methods, \textbf{10K} unpaired images for UDA methods)}                   \\ \hline
Baseline                 & -                  & \multicolumn{1}{c||}{\textbf{-}}                      & \multicolumn{1}{c|}{55.0}                                       & \multicolumn{1}{c|}{40.7}                                       & \multicolumn{1}{c|}{24.0}                                        & \multicolumn{1}{c|}{12.7}                                        & \multicolumn{1}{c||}{8.30}                                       & \multicolumn{1}{c|}{64.5}                                       & \multicolumn{1}{c|}{53.9}                                       & \multicolumn{1}{c|}{37.5}                                       & \multicolumn{1}{c|}{21.9}                                       & 14.8                                       \\
{CycleGAN}                 & {ICCV'17}                          & \multicolumn{1}{c||}{UIR}                    
 & \multicolumn{1}{c|}{46.5}        & \multicolumn{1}{c|}{36.2}         & \multicolumn{1}{c|}{23.1}         & \multicolumn{1}{c|}{14.2}         & \multicolumn{1}{c||}{\color[HTML]{3531ff}{\textbf{11.6 (3.3↑)}}}  & \multicolumn{1}{c|}{57.8}        & \multicolumn{1}{c|}{49.2}        & \multicolumn{1}{c|}{36.0}         & \multicolumn{1}{c|}{24.5}         & {\color[HTML]{3531ff}{\textbf{20.1 (5.3↑)}}}\\

UID-GAN                  & TBIOM'19                  & \multicolumn{1}{c||}{UIR}                    & \multicolumn{1}{c|}{39.0}                                       & \multicolumn{1}{c|}{22.3}                                       & \multicolumn{1}{c|}{8.10}                                        & \multicolumn{1}{c|}{3.60}                                        & \multicolumn{1}{c||}{2.30}                                       & \multicolumn{1}{c|}{50.1}                                       & \multicolumn{1}{c|}{33.5}                                       & \multicolumn{1}{c|}{13.6}                                       & \multicolumn{1}{c|}{5.90}                                       & 3.70                                       \\
DBGAN                    & CVPR'20                  & \multicolumn{1}{c||}{UIR}                    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{55.6 (0.6↑)}}}    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{44.7 (4.0↑)}}}    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{28.6 (4.6↑)}}}     & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{15.4 (2.7↑)}}}     & \multicolumn{1}{c||}{\color[HTML]{000000} 10.0}                           & \multicolumn{1}{c|}{63.9}                                       & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{56.8 (2.9↑)}}}    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{42.4 (4.9↑)}}}    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{25.3 (3.4↑)}}} & 17.1                                       \\
FCL-GAN                  & ACM MM'22                  & \multicolumn{1}{c||}{UIR}                    & \multicolumn{1}{c|}{54.5}                                       & \multicolumn{1}{c|}{42.2}                                       & \multicolumn{1}{c|}{25.7}                                        & \multicolumn{1}{c|}{13.5}                                        & \multicolumn{1}{c||}{5.70}                                       & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{64.9 (0.4↑)}}}    & \multicolumn{1}{c|}{55.7}                                       & \multicolumn{1}{c|}{40.7}                                       & \multicolumn{1}{c|}{24.9}                                       & 13.1                                       \\
CRNet                    & ACM MM'22                  & \multicolumn{1}{c||}{UIR}                    & \multicolumn{1}{c|}{22.9}                                       & \multicolumn{1}{c|}{17.6}                                       & \multicolumn{1}{c|}{6.40}                                        & \multicolumn{1}{c|}{2.90}                                        & \multicolumn{1}{c||}{3.90}                                       & \multicolumn{1}{c|}{32.7}                                       & \multicolumn{1}{c|}{27.2}                                       & \multicolumn{1}{c|}{11.9}                                       & \multicolumn{1}{c|}{5.70}                                       & 6.60                                       \\ 
DAN                     & PMLR'15                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{29.0}         & \multicolumn{1}{c|}{17.4}         & \multicolumn{1}{c|}{8.80}          & \multicolumn{1}{c|}{4.80}          & \multicolumn{1}{c||}{3.30}          & \multicolumn{1}{c|}{48.6}        & \multicolumn{1}{c|}{30.4}        & \multicolumn{1}{c|}{33.5}         & \multicolumn{1}{c|}{22.2}         & 11.6     \\

MDD                     & PMLR'19                  & \multicolumn{1}{c||}{UDA}                     & \multicolumn{1}{c|}{24.7}         & \multicolumn{1}{c|}{16.6}         & \multicolumn{1}{c|}{9.50}          & \multicolumn{1}{c|}{5.00}   & \multicolumn{1}{c||}{3.90}   & \multicolumn{1}{c|}{54.9}        & \multicolumn{1}{c|}{38.8}        & \multicolumn{1}{c|}{22.6}         & \multicolumn{1}{c|}{19.9}         & 14.6             \\


CGDM                     & CVPR'21                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{{\color[HTML]{000000} 39.7}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 28.6}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 14.8}}                 & \multicolumn{1}{c|}{3.00}                                        & \multicolumn{1}{c||}{1.80}                                       & \multicolumn{1}{c|}{{\color[HTML]{000000} 60.3}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 52.9}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 40.8}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 24.7}}    & {\color[HTML]{000000} 19.2}    \\ 

DAN-TransPar             & TIP'22                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{29.1}                                       & \multicolumn{1}{c|}{17.2}                                       & \multicolumn{1}{c|}{8.60}                                        & \multicolumn{1}{c|}{4.50}                                        & \multicolumn{1}{c||}{3.30}                                       & \multicolumn{1}{c|}{44.6}                                       & \multicolumn{1}{c|}{30.1}                                       & \multicolumn{1}{c|}{0.10}                                       & \multicolumn{1}{c|}{0.70}                                       & 9.30                                       \\
MDD-TransPar             & TIP'22                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{29.0}                                       & \multicolumn{1}{c|}{13.6}                                       & \multicolumn{1}{c|}{8.10}                                        & \multicolumn{1}{c|}{4.20}                                        & \multicolumn{1}{c||}{3.10}                                       & \multicolumn{1}{c|}{56.7}                                       & \multicolumn{1}{c|}{42.9}                                       & \multicolumn{1}{c|}{26.8}                                       & \multicolumn{1}{c|}{16.3}                                       & 12.0                                       \\


\hline
\textbf{UFEM (Ours)}                & \textbf{-}                  & \multicolumn{1}{c||}{\textbf{-}}                    & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \textbf{59.7 (4.7↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \textbf{50.6 (9.9↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \textbf{34.7 (10.7↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \textbf{22.8 (10.1↑)}}} & \multicolumn{1}{c||}{{\color[HTML]{fe0000} \textbf{15.3 (7.0↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \textbf{65.7 (1.3↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \textbf{58.2 (4.3↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \textbf{43.1 (5.6↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \textbf{26.7 (4.8↑)}}}                & {\color[HTML]{fe0000} \textbf{20.1 (5.3↑)}}   \\ \hline

\multicolumn{13}{c}{\cellcolor[HTML]{EAEAEA}\textbf{Degradation Type: Low Contrast} (\textbf{100} unpaired images for UFEM, \textbf{1200} unpaired images for UIR methods, \textbf{10K} unpaired images for UDA methods)}              \\ \hline
Baseline                 & -                  & \multicolumn{1}{c||}{\textbf{-}}                      & \multicolumn{1}{c|}{56.9}                                       & \multicolumn{1}{c|}{48.2}                                       & \multicolumn{1}{c|}{32.3}                                        & \multicolumn{1}{c|}{10.3}                                        & \multicolumn{1}{c||}{2.50}                                       & \multicolumn{1}{c|}{64.3}                                       & \multicolumn{1}{c|}{57.8}                                       & \multicolumn{1}{c|}{45.5}                                       & \multicolumn{1}{c|}{20.3}                                       & 5.40                                       \\
{CycleGAN}                 & {ICCV'17}                          & \multicolumn{1}{c||}{UIR}                    
& \multicolumn{1}{c|}{54.6}        & \multicolumn{1}{c|}{51.1}         & \multicolumn{1}{c|}{\color[HTML]{3531ff}{\textbf{47.0 (14.7↑)}}} & \multicolumn{1}{c|}{\color[HTML]{3531ff}{\textbf{31.9 (21.6↑)}}} & \multicolumn{1}{c||}{\color[HTML]{3531ff}{\textbf{12.4 (9.9↑)}}}  & \multicolumn{1}{c|}{63.4}        & \multicolumn{1}{c|}{60.5}        & \multicolumn{1}{c|}{\textcolor[RGB]{255,0,0}{\textbf{57.3 (11.8↑)}}} & \multicolumn{1}{c|}{\textcolor[RGB]{255,0,0}{\textbf{43.6 (23.3↑)}}} & \textcolor[RGB]{255,0,0}{\textbf{20.8 (15.4↑)}}                                      
\\
EnligntenGAN             & TIP'21                  & \multicolumn{1}{c||}{UIR}                    & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{58.7 (1.8↑)}}                           & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{52.5 (4.3↑)}}                           & \multicolumn{1}{c|}{\color[HTML]{000000} 34.8}                            & \multicolumn{1}{c|}{\color[HTML]{000000} 11.4}                            & \multicolumn{1}{c||}{\color[HTML]{000000} 2.70}                           & \multicolumn{1}{c|}{\color[HTML]{fe0000} \textbf{66.0 (1.7↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{60.7 (2.9↑)}}                           & \multicolumn{1}{c|}{47.3}                                       & \multicolumn{1}{c|}{22.3}                                       & 6.70                                       \\
Zero-DCE                 & CVPR'20                  & \multicolumn{1}{c||}{UIR}                    & \multicolumn{1}{c|}{21.1}                                       & \multicolumn{1}{c|}{11.3}                                       & \multicolumn{1}{c|}{6.50}                                        & \multicolumn{1}{c|}{1.50}                                        & \multicolumn{1}{c||}{0.50}                                       & \multicolumn{1}{c|}{27.7}                                       & \multicolumn{1}{c|}{16.0}                                       & \multicolumn{1}{c|}{9.00}                                       & \multicolumn{1}{c|}{1.90}                                       & 0.50                                       \\
ZeroDCE++                & TPAMI'21                  & \multicolumn{1}{c||}{UIR}                    & \multicolumn{1}{c|}{45.8}                                       & \multicolumn{1}{c|}{36.2}                                       & \multicolumn{1}{c|}{19.7}                                        & \multicolumn{1}{c|}{5.70}                                        & \multicolumn{1}{c||}{1.50}                                       & \multicolumn{1}{c|}{56.0}                                       & \multicolumn{1}{c|}{48.1}                                       & \multicolumn{1}{c|}{31.7}                                       & \multicolumn{1}{c|}{11.3}                                       & 2.70                                       \\
LE-GAN                   & KBS'22                  & \multicolumn{1}{c||}{UIR}                    & \multicolumn{1}{c|}{52.1}                                       & \multicolumn{1}{c|}{47.2}                                       & \multicolumn{1}{c|}{5.40}                                        & \multicolumn{1}{c|}{1.70}                                        & \multicolumn{1}{c||}{0.30}                                       & \multicolumn{1}{c|}{60.3}                                       & \multicolumn{1}{c|}{56.3}                                       & \multicolumn{1}{c|}{8.40}                                       & \multicolumn{1}{c|}{2.80}                                       & 0.50                                       \\ 
DAN                     & PMLR'15                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{23.8}         & \multicolumn{1}{c|}{17.5}         & \multicolumn{1}{c|}{11.0}         & \multicolumn{1}{c|}{3.50}          & \multicolumn{1}{c||}{1.00}          & \multicolumn{1}{c|}{53.3}        & \multicolumn{1}{c|}{35.9}        & \multicolumn{1}{c|}{43.6}         & \multicolumn{1}{c|}{23.7}         & 6.70                        \\ 
MDD                     & PMLR'19                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{21.9}         & \multicolumn{1}{c|}{13.3}         & \multicolumn{1}{c|}{8.50}          & \multicolumn{1}{c|}{3.80}          & \multicolumn{1}{c||}{1.50}          & \multicolumn{1}{c|}{53.7}        & \multicolumn{1}{c|}{45.3}        & \multicolumn{1}{c|}{31.3}         & \multicolumn{1}{c|}{20.9}         & 8.20                        \\ 
CGDM                     & CVPR'21                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{44.5}                                       & \multicolumn{1}{c|}{40.4}                                       & \multicolumn{1}{c|}{33.3}                                        & \multicolumn{1}{c|}{7.80}                                        & \multicolumn{1}{c||}{1.70}                                       & \multicolumn{1}{c|}{61.6}                                       & \multicolumn{1}{c|}{58.5}                                       & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{53.4 (7.9↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{34.3 (14.0↑)}}                       & \color[HTML]{3531ff} \textbf{12.0 (6.6↑)}                        \\ 

DAN-TransPar             & TIP'22                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{23.4}                                       & \multicolumn{1}{c|}{17.7}                                       & \multicolumn{1}{c|}{10.4}                                        & \multicolumn{1}{c|}{3.20}                                        & \multicolumn{1}{c||}{1.10}                                       & \multicolumn{1}{c|}{45.6}                                       & \multicolumn{1}{c|}{48.0}                                       & \multicolumn{1}{c|}{11.9}                                       & \multicolumn{1}{c|}{0.10}                                       & 5.40                                       \\
MDD-TransPar             & TIP22                  & \multicolumn{1}{c||}{UDA}                    & \multicolumn{1}{c|}{19.1}                                       & \multicolumn{1}{c|}{11.6}                                       & \multicolumn{1}{c|}{7.40}                                        & \multicolumn{1}{c|}{3.20}                                        & \multicolumn{1}{c||}{1.30}                                       & \multicolumn{1}{c|}{57.0}                                       & \multicolumn{1}{c|}{41.7}                                       & \multicolumn{1}{c|}{26.2}                                       & \multicolumn{1}{c|}{15.8}                                       & 5.70                                       \\

\hline
\textbf{UFEM (Ours)}                & \textbf{-}                  & \multicolumn{1}{c||}{\textbf{-}}                    & \multicolumn{1}{c|}{\color[HTML]{fe0000} \textbf{62.8 (5.9↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{fe0000} \textbf{58.8 (10.6↑)}}                       & \multicolumn{1}{c|}{\color[HTML]{fe0000} \textbf{53.0 (20.7↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{fe0000} \textbf{32.0 (21.7↑)}}                        & \multicolumn{1}{c||}{\color[HTML]{fe0000} \textbf{14.5 (12.0↑)}}                       & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{65.0 (0.7↑)}}                           & \multicolumn{1}{c|}{\color[HTML]{fe0000} \textbf{60.8 (3.0↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{000000} 48.5}                           & \multicolumn{1}{c|}{\color[HTML]{000000} 23.2}                           & {\color[HTML]{000000} 8.40}          \\ \Xhline{1.5pt}
\end{tabular}
}
\end{table*}

==> Table/ClassificationSynthetic.tex <==

\begin{table*}[htbp]
\small
    \centering
    \caption{The comparisons of our proposed DCP with Unsupervised Image Restoration (UIR) and Unsupervised Domain Adaption (UDA) methods under two different degradation types, \emph{i.e.}, Fog, and Motion blur. Each corruption type contains 5 severity levels.}
    \label{tab:cls_syn}
    \resizebox{\textwidth}{!}{
    \renewcommand\arraystretch{1.2}
    \begin{tabular}{lccccccccccc}
    \Xhline{1.5pt}
                                 & \multicolumn{1}{c||}{}                                
                                  & \multicolumn{5}{c||}{\textbf{Top-1 Accuracy of VGG16 (\%)}}           & \multicolumn{5}{c}{\textbf{Top-1 Accuracy of ResNet50 (\%)}}                                                                                                                                                                                                                                                     \\ 
                                  \cline{3-12} 

\multirow{-2}{*}{\textbf{Method}} & \multicolumn{1}{c||}{\multirow{-2}{*}{\textbf{Venue}}}  & \multicolumn{1}{c|}{\textbf{Level-1}}                           & \multicolumn{1}{c|}{\textbf{Level-2}}                           & \multicolumn{1}{c|}{\textbf{Level-3}}                            & \multicolumn{1}{c|}{\textbf{Level-4}}                            & \multicolumn{1}{c||}{\textbf{Level-5}}                           & \multicolumn{1}{c|}{\textbf{Level-1}}                           & \multicolumn{1}{c|}{\textbf{Level-2}}                           & \multicolumn{1}{c|}{\textbf{Level-3}}                           & \multicolumn{1}{c|}{\textbf{Level-4}}                           & \textbf{Level-5}                           \\ \hline
\multicolumn{12}{c}{\textbf{Degradation Type: Fog} (\textbf{100} unpaired images for DCP, \textbf{1200} unpaired images for UIR methods, \textbf{10K} unpaired images for UDA methods)}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
Baseline                & \multicolumn{1}{c||}{\textbf{-}}                      & \multicolumn{1}{c|}{53.6}                                       & \multicolumn{1}{c|}{46.1}                                       & \multicolumn{1}{c|}{36.7}                                        & \multicolumn{1}{c|}{31.6}                                        & \multicolumn{1}{c||}{17.5}                                       & \multicolumn{1}{c|}{61.4}                                       & \multicolumn{1}{c|}{55.3}                                       & \multicolumn{1}{c|}{46.2}                                       & \multicolumn{1}{c|}{39.6}                                       & 23.7                                       \\
YOLY \cite{li2021you}                     & \multicolumn{1}{c||}{IJCV'21}                   & \multicolumn{1}{c|}{57.2}                                       & \multicolumn{1}{c|}{52.6}                                       & \multicolumn{1}{c|}{44.0}                                        & \multicolumn{1}{c|}{36.6}                                        & \multicolumn{1}{c||}{20.4}                                       & \multicolumn{1}{c|}{63.1}                                       & \multicolumn{1}{c|}{58.0}                                       & \multicolumn{1}{c|}{49.4}                                       & \multicolumn{1}{c|}{41.9}                                       & 25.4                                       \\
RefineDNet \cite{zhao2021refinednet}              & \multicolumn{1}{c||}{TIP'21}                    & \multicolumn{1}{c|}{58.3}                                       & \multicolumn{1}{c|}{54.8}                                       & \multicolumn{1}{c|}{48.4}                                        & \multicolumn{1}{c|}{42.1}                                        & \multicolumn{1}{c||}{\color[HTML]{3531ff} \textbf{27.6 (10.1↑)}}                          & \multicolumn{1}{c|}{62.2}                                       & \multicolumn{1}{c|}{58.7}                                       & \multicolumn{1}{c|}{51.7}                                       & \multicolumn{1}{c|}{45.9}                                       & 31.9                                       \\
CGDM \cite{du2021cross}                     & \multicolumn{1}{c||}{CVPR'21}      & \multicolumn{1}{c|}{43.7}                                       & \multicolumn{1}{c|}{40.5}                                       & \multicolumn{1}{c|}{36.1}                                        & \multicolumn{1}{c|}{33.0}                                        & \multicolumn{1}{c||}{23.4}                                       & \multicolumn{1}{c|}{60.5}                                       & \multicolumn{1}{c|}{57.3}                                       & \multicolumn{1}{c|}{54.1}                                       & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{50.6 (11.0↑)}}                          & \color[HTML]{3531ff} \textbf{40.9 (17.2↑)}                          \\ 
{SNSPGAN \cite{wang2022cycle}}                & \multicolumn{1}{c||}{ITS'22}                    
& \multicolumn{1}{c|}{51.0}                           & \multicolumn{1}{c|}{42.5}                      
& \multicolumn{1}{c|}{32.1}                           & \multicolumn{1}{c|}{28.4}                           
& \multicolumn{1}{c||}{15.3}                          & \multicolumn{1}{c|}{59.2}                      
& \multicolumn{1}{c|}{52.2}                           & \multicolumn{1}{c|}{41.7}                           
& \multicolumn{1}{c|}{36.6}                                       & {21.2}                                     
\\

D4 \cite{yang2022D4}                       & \multicolumn{1}{c||}{CVPR'22}                 & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{60.2 (6.6↑)}}                           & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{56.2 (10.1↑)}}                          & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{48.5 (11.8↑)}}                           & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{42.2 (10.6↑)}}                           & \multicolumn{1}{c||}{18.3}                                       & \multicolumn{1}{c|}{\color[HTML]{fe0000} \textbf{66.1 (4.7↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{62.1 (6.8↑)}}                           & \multicolumn{1}{c|}{\color[HTML]{3531ff} \textbf{54.2 (8.0↑)}}                           & \multicolumn{1}{c|}{47.4}                                       & 24.3                                       \\

DAN-TransPar  \cite{han2022learning}            & \multicolumn{1}{c||}{TIP'22}          & \multicolumn{1}{c|}{23.2}                                       & \multicolumn{1}{c|}{17.7}                                       & \multicolumn{1}{c|}{13.2}                                        & \multicolumn{1}{c|}{11.4}                                        & \multicolumn{1}{c||}{5.90}                                       & \multicolumn{1}{c|}{40.6}                                       & \multicolumn{1}{c|}{42.7}                                       & \multicolumn{1}{c|}{29.2}                                       & \multicolumn{1}{c|}{35.0}                                       & 0.10                                       \\
MDD-TransPar \cite{han2022learning}             & \multicolumn{1}{c||}{TIP'22}    & \multicolumn{1}{c|}{20.8}                                       & \multicolumn{1}{c|}{16.7}                                       & \multicolumn{1}{c|}{13.1}                                        & \multicolumn{1}{c|}{13.0}                                        & \multicolumn{1}{c||}{8.60}                                       & \multicolumn{1}{c|}{53.4}                                       & \multicolumn{1}{c|}{39.9}                                       & \multicolumn{1}{c|}{35.5}                                       & \multicolumn{1}{c|}{33.8}                                       & 27.1                                       \\
SLP \cite{ling2023single}                     & \multicolumn{1}{c||}{TIP'23}    & \multicolumn{1}{c|}{58.9}                                       & \multicolumn{1}{c|}{55.2}                                       & \multicolumn{1}{c|}{47.8}                                        & \multicolumn{1}{c|}{39.8}                                        & \multicolumn{1}{c||}{24.2}                                       & \multicolumn{1}{c|}{64.5}                                       & \multicolumn{1}{c|}{60.7}                                       & \multicolumn{1}{c|}{53.2}                                       & \multicolumn{1}{c|}{45.6}                                       & 30.4                                       \\
\hline

\cellcolor[HTML]{EAEAEA}\textbf{DCP (Ours)}               & \multicolumn{1}{c||}{\cellcolor[HTML]{EAEAEA}\textbf{-}}                    & \multicolumn{1}{c|}{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{61.7 (8.1↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{59.2 (13.1↑)}}                       & \multicolumn{1}{c|}{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{56.4 (19.7↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{53.2 (21.6↑)}}                        & \multicolumn{1}{c||}{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{43.6 (26.1↑)}}                       & \multicolumn{1}{c|}{\color[HTML]{3531ff} \cellcolor[HTML]{EAEAEA}\textbf{64.4 (3.0↑)}}                           & \multicolumn{1}{c|}{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{62.3 (7.1↑)}}                        & \multicolumn{1}{c|}{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{57.1 (10.9↑)}}                       & \multicolumn{1}{c|}{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{52.4 (12.8↑)}}                       & \color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{42.0 (18.1↑)}                       \\ \hline


\multicolumn{12}{c}{\textbf{Degradation Type: Motion blur} (\textbf{100} unpaired images for DCP, \textbf{1200} unpaired images for UIR methods, \textbf{10K} unpaired images for UDA methods)}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
Baseline                  & \multicolumn{1}{c||}{\textbf{-}}                      & \multicolumn{1}{c|}{55.0}                                       & \multicolumn{1}{c|}{40.7}                                       & \multicolumn{1}{c|}{24.0}                                        & \multicolumn{1}{c|}{12.7}                                        & \multicolumn{1}{c||}{8.30}                                       & \multicolumn{1}{c|}{64.5}                                       & \multicolumn{1}{c|}{53.9}                                       & \multicolumn{1}{c|}{37.5}                                       & \multicolumn{1}{c|}{21.9}                                       & 14.8                                       \\
UID-GAN \cite{lu2019uid}                 & \multicolumn{1}{c||}{TBIOM'19}                    & \multicolumn{1}{c|}{39.0}                                       & \multicolumn{1}{c|}{22.3}                                       & \multicolumn{1}{c|}{8.10}                                        & \multicolumn{1}{c|}{3.60}                                        & \multicolumn{1}{c||}{2.30}                                       & \multicolumn{1}{c|}{50.1}                                       & \multicolumn{1}{c|}{33.5}                                       & \multicolumn{1}{c|}{13.6}                                       & \multicolumn{1}{c|}{5.90}                                       & 3.70                                       \\
DBGAN \cite{zhang2020deblurring}                   & \multicolumn{1}{c||}{CVPR'20}                   & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{55.6 (0.6↑)}}}    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{44.7 (4.0↑)}}}    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{28.6 (4.6↑)}}}     & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{15.4 (2.7↑)}}}     & \multicolumn{1}{c||}{\color[HTML]{3531ff} \textbf{10.0 (1.7↑)}}                           & \multicolumn{1}{c|}{63.9}                                       & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{56.8 (2.9↑)}}}    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{42.4 (4.9↑)}}}    & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{25.3 (3.4↑)}}} & 17.1                                       \\
CGDM \cite{du2021cross}                     & \multicolumn{1}{c||}{CVPR'21}                    & \multicolumn{1}{c|}{{\color[HTML]{000000} 39.7}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 28.6}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 14.8}}                 & \multicolumn{1}{c|}{3.00}                                        & \multicolumn{1}{c||}{1.80}                                       & \multicolumn{1}{c|}{{\color[HTML]{000000} 60.3}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 52.9}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} 40.8}}                & \multicolumn{1}{c|}{{\color[HTML]{000000} {24.7}}}    & {\color[HTML]{3531ff} \textbf{19.2 (4.4↑)}}    \\ 
FCL-GAN \cite{zhao2022fcl}                 & \multicolumn{1}{c||}{ACM MM'22}                    & \multicolumn{1}{c|}{54.5}                                       & \multicolumn{1}{c|}{42.2}                                       & \multicolumn{1}{c|}{25.7}                                        & \multicolumn{1}{c|}{13.5}                                        & \multicolumn{1}{c||}{5.70}                                       & \multicolumn{1}{c|}{{\color[HTML]{3531ff} \textbf{64.9 (0.4↑)}}}    & \multicolumn{1}{c|}{55.7}                                       & \multicolumn{1}{c|}{40.7}                                       & \multicolumn{1}{c|}{24.9}                                       & 13.1                                       \\
CRNet \cite{zhao2022crnet}                   & \multicolumn{1}{c||}{ACM MM'22}                  & \multicolumn{1}{c|}{22.9}                                       & \multicolumn{1}{c|}{17.6}                                       & \multicolumn{1}{c|}{6.40}                                        & \multicolumn{1}{c|}{2.90}                                        & \multicolumn{1}{c||}{3.90}                                       & \multicolumn{1}{c|}{32.7}                                       & \multicolumn{1}{c|}{27.2}                                       & \multicolumn{1}{c|}{11.9}                                       & \multicolumn{1}{c|}{5.70}                                       & 6.60                                       \\





DAN-TransPar \cite{han2022learning}            & \multicolumn{1}{c||}{TIP'22}                    & \multicolumn{1}{c|}{29.1}                                       & \multicolumn{1}{c|}{17.2}                                       & \multicolumn{1}{c|}{8.60}                                        & \multicolumn{1}{c|}{4.50}                                        & \multicolumn{1}{c||}{3.30}                                       & \multicolumn{1}{c|}{44.6}                                       & \multicolumn{1}{c|}{30.1}                                       & \multicolumn{1}{c|}{0.10}                                       & \multicolumn{1}{c|}{0.70}                                       & 9.30                                       \\
MDD-TransPar \cite{han2022learning}            & \multicolumn{1}{c||}{TIP'22}                  & \multicolumn{1}{c|}{29.0}                                       & \multicolumn{1}{c|}{13.6}                                       & \multicolumn{1}{c|}{8.10}                                        & \multicolumn{1}{c|}{4.20}                                        & \multicolumn{1}{c||}{3.10}                                       & \multicolumn{1}{c|}{56.7}                                       & \multicolumn{1}{c|}{42.9}                                       & \multicolumn{1}{c|}{26.8}                                       & \multicolumn{1}{c|}{16.3}                                       & 12.0                                       \\
{-}                  & \multicolumn{1}{c||}{-}                    
& \multicolumn{1}{c|}{-}                           & \multicolumn{1}{c|}{-}                          
& \multicolumn{1}{c|}{-}                           & \multicolumn{1}{c|}{-}                           
& \multicolumn{1}{c||}{-}                          & \multicolumn{1}{c|}{-}                      
& \multicolumn{1}{c|}{-}                           & \multicolumn{1}{c|}{-}                           
& \multicolumn{1}{c|}{-}                                       & {-}                                     
\\

\hline
\cellcolor[HTML]{EAEAEA}\textbf{DCP (Ours)}        & \multicolumn{1}{c||}{\cellcolor[HTML]{EAEAEA}\textbf{-}}                    & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{59.7 (4.7↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{50.6 (9.9↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{34.7 (10.7↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{22.8 (10.1↑)}}} & \multicolumn{1}{c||}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{15.3 (7.0↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{65.7 (1.3↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{58.2 (4.3↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{43.1 (5.6↑)}}} & \multicolumn{1}{c|}{{\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{26.7 (4.8↑)}}}                & {\color[HTML]{fe0000} \cellcolor[HTML]{EAEAEA}\textbf{20.1 (5.3↑)}} \\ \Xhline{1.5pt}
\end{tabular}

}
\end{table*}

